Regularity as Regularization: Smooth and Strongly Convex Brenier Potentials in Optimal Transport

Estimating Wasserstein distances between two high-dimensional densities suffers from the curse of dimensionality: one needs an exponential (wrt dimension) number of samples to ensure that the distance between two empirical measures is comparable to the distance between the original densities. Therefore, optimal transport (OT) can only be used in machine learning if it is substantially regularized. On the other hand, one of the greatest achievements of the OT literature in recent years lies in regularity theory: Caffarelli showed that the OT map between two well behaved measures is Lipschitz, or equivalently when considering 2-Wasserstein distances, that Brenier convex potentials (whose gradient yields an optimal map) are smooth. We propose in this work to draw inspiration from this theory and use regularity as a regularization tool. We give algorithms operating on two discrete measures that can recover nearly optimal transport maps with small distortion, or equivalently, nearly optimal Brenier potentials that are strongly convex and smooth. The problem boils down to solving alternatively a convex QCQP and a discrete OT problem, granting access to the values and gradients of the Brenier potential not only on sampled points, but also out of sample at the cost of solving a simpler QCQP for each evaluation. We propose algorithms to estimate and evaluate transport maps with desired regularity properties, benchmark their statistical performance, apply them to domain adaptation and visualize their action on a color transfer task.

==> sections/highdimension.tex <==
\section{Semidefinite Relaxations in the Higher-dimensional Case}
%add algo box
%\MC{
%\begin{enumerate}
%    \item On pose le problème comme un QCQP (minimisation alternée entre transport et QCQP non convexe) avec des contraintes $(i,j)$ quand $i\sim j$ ($x_i$ et $x_j$ sont connectés)
%    \item Le QCQP non convexe peut se lifter en SDP qui est tight si 2(n+m) < d.
%    \item On explique le lifting, et surtout on montre que dans le cas où le graphe n'est pas connecté (k-means) on parallélise les SDPs.
%\end{enumerate}
%}

In this section, we provide algorithms to compute a SSNB potential in dimension $d \geq 2$ when $\mu,\nu$ are discrete measures. In order to solve Problem~\eqref{eqn:SSNB}, we will alternate between minimizing over $(z_1, \ldots, z_n, u)$ and computing a coupling $P$ solving the OT problem. The OT computation can be efficiently carried out using Sinkhorn's algorithm~\cite{CuturiSinkhorn}. The other minimization is a convex QCQP, separable in $K$ smaller convex QCQP.

\begin{wrapfigure}{r}{0.4\textwidth}
    \vskip-.5cm
    \begin{algorithm}[H]
         Initialize $z_1, \ldots, z_n \in \Rd$\\
         \Repeat{convergence}{
            $C \leftarrow \left( \|z_i - y_j\|^2 \right)_{ij}$ \\
            $P \leftarrow \text{OT}(a, b, C)$ \\
            \For{$k=1,\ldots,K$} {
                $\{z_i \,|\, i\in I_k\} \leftarrow \text{SDP}_k(P)$\\
            }
         }
         \caption{Alternate Minimization for SSNB computation. $\text{SDP}_k(P)$ implements a SDP solver for problem~\eqref{opti:SDP}.}\label{algo:SDP}
        \end{algorithm}
    \vskip-.7cm
\end{wrapfigure}

\textbf{SDP relaxation}
Let $k \in \range{K}$ and write $n_k = |E_k|$. For $z_1, \ldots, z_{n_k} \in \Rd$, we define $G \in \R^{(2n_k+m) \times (2n_k+m)}$ to be the Gram matrix associated with points $x_i \in E_k$, $z_1, \ldots, z_{n_k}$ and $y_1, \ldots, y_m$. To simplify notations, we will write $G(\alpha_i, \beta_j)$ for the coefficient in $G$ corresponding to $\dotp{\alpha_i}{\beta_j}$ where $\alpha, \beta \in \{x,y,z\}$. 

% ======== From Alex ========
To relax the original problem, we can do a change of variables, introducing the matrix variables $Z_i=z_iz_i^T$. This is of course a nonconvex constraint in $(z_i,Z_i)$ but we can relax it to $z_iz_i^T \preceq Z_i$ which is a Schur complement. By construction, we also have $\tr(Z_i)=G(z_i,z_i)$, hence $\|z_i\|_2^2 \leq G(z_i,z_i)$.

The locations $x_i \in E_k, y_1,\ldots,y_m$ are known and fixed, the terms $G(y_j,z_i)$ and $G(x_j,z_i)$ are linear, written $G(y_j,z_i)=z_i^Ty_j$ and $G(x_j,z_i)=z_i^Tx_j$ for $z_i\in \Rd$. Overall, for a fixed transport plan $P \in \mathcal{U}(a,b)$, we have to solve the following SDPs (one for each $k \in \range{K}$):
\begin{align}\label{opti:SDP}
    &\min_{G \succeq 0, u \in \R^{I_k}}
    \left\{ \sum_{i \in I_k} \sum_{j=1}^m P_{i,j} \left[ G(y_j,y_j) + G(z_i,z_i) - 2G(y_j,z_i) \right]
    \right\}\\
    & \textrm{s.t.  } \forall i,j \in I_k,\, u_i \geq u_j + G(z_j, x_i) - G(z_j, x_j) \nonumber \\
    & \qquad \qquad \qquad + \frac{1}{2(1-\scvx/L)} \left( 
    \frac{1}{L} \left[ G(z_i, z_i) + G(z_j, z_j) - 2G(z_i, z_j) \right] \right. \nonumber \\
    & \left. \qquad \qquad \qquad + \scvx \|x_i - x_j\|^2
    - 2 \frac{\scvx}{L} \left[ G(z_j, x_j) - G(z_j, x_i) - G(z_i, x_j) + G(z_i, x_i) \right]
    \vphantom{\frac{1}{2(1-\scvx/L)}}\right)\nonumber\\
    & \qquad \forall i \in I_k,\, \|z_i\|_2^2 \leq G(z_i,z_i),\, \forall j\in\range{m},\, G(y_j,z_i)=z_i^T y_j,\, G(x_j,z_i)=z_i^T x_j.\nonumber
\end{align}

This semidefinite relaxation will be tight when the ambient dimension $d$ is of the same order as the number of points \citep{taylor2017smooth}. When $d$ is smaller, there is a gap between the optimum of the SDP and that of the QCQP, and we need to find (or approximate) a low rank solution.


% AA: CHECK. Additional constraints xx^T \preceq X should be redundant, summarized as $\|g_i\|_2\leq G(z_i,z_i)$.


%\textbf{L-BFGS} We can also run a L-BFGS descent on the objective, adding a log barrier for the constraints.


==> sections/rebuttal.tex <==
\newpage

\section{Rebuttal}

\subsection{Reviewer 1}
\textit{1. Contributions: Please list three things this paper contributes (e.g., theoretical, methodological, algorithmic, empirical contributions; bridging fields; or providing an important critical analysis). For each contribution, briefly state the level of significance (i.e., how much impact will this work have on researchers and practitioners in the future?). If you cannot think of three things, please explain why. Not all good papers will have three contributions.}
\begin{itemize}
    \item The authors consider the optimal transportation problem, and propose to regularize the transport map between two measures by imposing certain (local) Lipschitzness constraints on it.
    \item They take an optimization perspective and propose a non-convex program that can solve this problem optimally. This algorithm amounts to performing isotonic regression in dimension 1.
    \item In general dimensions, some SDP-based heuristics are designed and evaluated on a color transfer task. They are able to show that setting the regularizer appropriately leads to qualitatively different results on the task, thus providing additional flexibility on top of traditional OT.
\end{itemize}{}

\textit{2. Detailed comments: Please provide a thorough review of the submission, including its originality, quality, clarity, and significance. Hover over the "?" next to this prompt to see a brief description of these metrics.}

Clarity: Results and implications are clearly stated and discussed. Some specific comments:

There seems to be some confusion throughout in the exposition about the “empirical” distribution and the “population” distribution. Indeed, \IMP{Brenier’s theorem (or even Theorem 1 of the paper) only guarantees the existence of a transport map for pairs of measures with finite second moments and *without atoms*.} However, the authors go on to use Theorem 1 as justification for carrying out OT on *discrete* measures. I presume the intention here was to say that OT is actually carried out on a *finite sample* from the population, from which the empirical distribution was constructed (and is therefore necessarily discrete). If so, it would be good to be explicit about this distinction, since structural results from OT are used as justification for the authors’ approach.
\REP{Indeed, it is not strictly speaking Brenier theorem. But if $f$ is convex and $\mu$ has a finite second-order moment, $\nabla f$ is optimal between $\mu$ and ${\nabla f}_\sharp\mu$ with no other assumption on $\mu$ (see Theorem 1.48 in Santambrogio).}

line 160: the letter “l” is missing from general

Originality: While the idea of imposing smoothness on the optimal transport map is a natural one, the authors deserve credit for proposing it as a regularization mechanism and trying their approach on an application. A particular question regarding some concurrent work:

The paper [1] considers the statistical aspects of finding transport maps from samples. (Global) Smoothness and strong convexity are also imposed as natural regularization mechanisms here, and rates are derived for a certain estimator of the map that uses the semi-dual optimization problem. Computational issues are not considered in [1], however. It would be good for the authors to compare and contrast their optimization formulation with [1]; in particular, \IMP{is it true that the statistical results of [1] carry over to the estimator proposed in this paper, at least when the partition $E_k$ consists of a single element?} Or are these fundamentally different approaches?
\REP{[1] Only considers measures over the hypercube $[0,1]^d$. In this case the lower bound holds: SSNB estimator in the worst case cannot beat the lower bound of $n^{-1/d}$. But empirically, the constant is much better, which is not analyzed in [1] and is of utmost importance in practice.}

Significance: OT is an interesting emerging area, and this paper makes a nice contribution to imposing regularization while using it. It also raises some interesting computational questions.

Quality: The prose of a reasonably high quality, and the proofs are correct as far as I can tell. The lack of a provably efficient algorithm (in general dimensions) is a drawback, but the application to real data is interesting, and likely to spur further research on this problem. \REP{In fact convex QCQP alternated with OT : local min.} \IMP{I would have appreciated a more detailed setup of the experiments though.}
\REP{New graphs + new exp in Domain Adaptation ?}

[1]: Hütter, J. C., \& Rigollet, P. (2019). Minimax rates of estimation for smooth optimal transport maps. arXiv preprint arXiv:1905.05828.

\textit{5. Improvements: What would the authors have to do for you to increase your score?}
While the idea is a natural one, the lack of a provable algorithm to perform this task merits a weak accept decision in my opinion.


\subsection{Reviewer 2}

\textit{1. Contributions: Please list three things this paper contributes (e.g., theoretical, methodological, algorithmic, empirical contributions; bridging fields; or providing an important critical analysis). For each contribution, briefly state the level of significance (i.e., how much impact will this work have on researchers and practitioners in the future?). If you cannot think of three things, please explain why. Not all good papers will have three contributions.}
\begin{itemize}
    \item 1) The authors present a modification of the classic OT problem by restricting the space of transport plans to those with bounded distortion (L-Lipschitz with l-strongly convex Brenier potentials). Recent results from first order methods are applied directly to see that this is a QCQP optimization problem (in the case of discrete measures). This new perspective could be quite useful for particular application scenarios, as shown in the experiments, and is an interesting new perspective for the machine learning community.
    \item 2) For the univariate case, the problem is shown to be equivalent to optimizing $L^2$ (w.r.t source measure $\mu$) distance from the barycentric projection of the optimal coupling. This is the Lipschitz isotonic regression problem, and a simple algorithm is proposed. This is an interesting tie-in to a different applied problem that I have not heard of before, and should be interesting to the broader machine learning community, I imagine.
    \item 3) For the multivariate case, an alternating minimization approach is suggested, with Sinkhorn OT steps alternated with an SDP relaxation. This approach is utilized to propose a Wasserstein distance estimator based on empirical samples, and is also used in experiments on color transfer. These are good first steps to solving this problem computationally and will spur further investigation into solving this modified OT problem.
\end{itemize}


\textit{2. Detailed comments: Please provide a thorough review of the submission, including its originality, quality, clarity, and significance. Hover over the "?" next to this prompt to see a brief description of these metrics.}

The article provides a clear proposal for a modified OT problem, where one enforces regularity of the transport map. I did not read every proof in the supplemental material, but the analysis seems quite careful and some nontrivial algorithms are proposed.

The main knock against this work would be that \IMP{the exciting application of a more quickly convergent estimator is not fully explored}, and the color transfer application is merely a proof-of-principle that shows expected behavior based on variation of l and L. In fact, computationally, \IMP{it is not clear to me that the SDP would be practically efficient in many cases, so I'm unsure that the proposed methods are immediately useful as is}. However, I'm sure that other researchers might take up this pursuit and explore this interesting idea for modification of the classic OT problem.
\REP{Domain Adaptation + some new experiment with statistics ?}


\textit{5. Improvements: What would the authors have to do for you to increase your score?}
The faster convergence of the proposed estimator is quite exciting, so it'd be nice if this was explored further. Runtimes would be useful to note in this case.

Additional applications would bolster the impact of the work and motivate others to investigate this problem.
\REP{New exp ?}

Small things:

Line 43 (and elsewhere): presumably it should be $e^{-V}$ so that one has finite measure? \REP{No.}
Fig. 3: colors are hard to distinguish; yellow line is hard to even see \REP{Will be changed.}
Line 210: $E_k$ -> $I_k$, presumably?
Fig. 5: Would be less confusing to use $\times$ for the approximate W values \REP{Will be changed.}


\subsection{Reviewer 3}

\textit{1. Contributions: Please list three things this paper contributes (e.g., theoretical, methodological, algorithmic, empirical contributions; bridging fields; or providing an important critical analysis). For each contribution, briefly state the level of significance (i.e., how much impact will this work have on researchers and practitioners in the future?). If you cannot think of three things, please explain why. Not all good papers will have three contributions.}

The focus of this paper is to propose an optimization-based approach to estimate the solution of the optimal transport problem. The claimed contributions in the paper are the following:

(C1) To introduce a relaxed optimal transport problem in which the so-called Brenier potential function is restricted to the L-smooth and $\ell$-strongly convex function. It is also claimed that this class of problems falls into the category of (non-convex) QCQP. 

(C2) To show that the problem in the univariate case (distributions supported on R) can be exactly reformulated as a convex optimization problem. 

(C3) To introduce an SDP relaxation of the resulting QCQP problem.

(C4) To implement the proposed solution in a color transfer application. 

The paper reads well and the mathematical arguments are formalized precisely. The optimal transport is an important problem, and an efficient approximation, which is the main motivation of this study, would have a remarkable impact in many areas. While I enjoy reading this paper, it seems the proposed solution has several shortcomings which I will explain in the "Detailed comments".
\REP{We do not seek an efficient approximation, but wish to regularize OT.}

\textit{2. Detailed comments: Please provide a thorough review of the submission, including its originality, quality, clarity, and significance. Hover over the "?" next to this prompt to see a brief description of these metrics.}

\#\#\# Problem description and proposed solution: 
The main focus of the paper is the optimal transport problem, particularly the Monge version, as defined in the equation after line 73. To the best of my understanding, the following steps is the summary of the proposed approximation procedure: \REP{Not an approximation procedure !}

(S1) Define a relaxed version (Definition 1, line 118) where the Brenier potential is confined to an ell-L regular convex function. 

(S2) Restrict the transportation cost in the previous step to be evaluated only at certain prespecified locations "$x_i$". In other words, the marginal "$\mu$" is treated as an empirical distribution (line 135).

(S3) Translate the modified problem in Definition 2 to a finite convex optimization in (1) (Theorem 2, line 148).

(S4) Propose an alternating procedure by fixing the variables "$P_ij$" and optimizing over the variables "$z_i$" and "$u_i$", which is a non-convex QCQP, and vice versa, that is, fixing "$z_i$" and "$u_i$" and optimizing over "$P_ij$", which is a linear program (Algorithm 1, lines 211-221)

(S5) Further relax the QCQP program by replacing the bilinear terms via an SCP approximation (program (4) after line 225). 

\#\#\# Major comments: 
\IMP{(1) Strictly speaking, claim (C1) regarding QCQP reformulation seems to be incorrect. This only holds if the resulting cost is only evaluated at the particular given locations of the marginal mu. Therefore, if I understand correctly, when the marginal $\mu$ is a continuous distribution, the program (1) in Theorem 2 is not exactly a reformulation of the optimal transport in Definition 1. This is transparent in the paper.}
\REP{As stated in line 135, we only consider discrete measures in the algorithms. (Maybe add something about the statistical setting since he did not understand what we are doing).}

\IMP{(2) Regarding the claim (C3), the argument is incomplete since the SDP relaxation is not the only part of the relaxation. It seems that there is also a bi-linearity between the variable "P" and others decision variables that the authors treat via an alternating optimization procedure. Thus, the error caused by this alternatin procedure, as described in (S4), seems to be neglected. This introduces another level of approximation error and is not mentioned explicitly in the paper.}
\REP{In fact QCQP is convex. Alternating minimization : should converge to a local min, cf. k-means, plus Sinkhorn add strong convexity for OT.}

\IMP{(3) One of the main motivations of this paper is the computational complexity of the original problem of the optimal transport. Given this, it would ideally be expected that the complexity of the proposed approximation method is also formally discussed. This is, in my opinion, necessariy to judge the validity of authors' claim on reducing the computational burden.}
\REP{Our motivation is not the computational complexity of computing OT. We show empirically that the statistical \textbf{sample complexity} seem to be better. Even if computational complexity is large, a small number of samples in our framework beats a large amount of samples in classical OT framework. + see answer to reviewer 2 regarding JC+Philippe's paper.}

\#\#\# Other comments: 
(1) It remains unclear to me how one can assess the quality of the proposed solution given the approximation error introduced through each and ever step of (S1)-(S5).
\REP{See QCQP is indeed convex + alternate min -> local min}

(2) The "color transfer" application mentioned in (C4) is indeed interesting but tt would also be very good if the authors could provide some intuitive explanation on how the regularity constants "$\ell$" and "L" can be interpreted in the color transfer application. 
\REP{Intuitive explanation is written in the paper, Fig.5 caption.} As of now, the impact of the parameter is only experimentally verified. \REP{If real map has regularity (l,L), then the estimator is consistent. Otherwise it is not, see Fig.3.}

Minor comments and typos:

(1) I think it is "an" L-smooth function, instead of "a" L-smooth function. Similar comments for the following: 
- "an" SDP (lines 57, 221) 
- "an" SSNB (lines 124, 131, 175) 
Please check the paper and the supplementary for these issues. 

(2) line 17: ... can be lifted "to" a semidefinite ... ;

(3) line 47: ... should be "regularized" into an algorithmic ... ;

(4) line 51: ... because "it" nearly transport ... ;

(5) line 160: ... is not optimal in "general" ... ;

(5) line 255: ... can "be" estimated ... .


\textit{5. Improvements: What would the authors have to do for you to increase your score?}
In the section "detailed comments", I mentioned three "major" and two "other" comments. I am open to change my overall score based on the authors' response to these comments.
